A Survey of Models for Cognitive Diagnosis: New Developments and Future Directions

Cognitive diagnosis has been developed for decades as an effective measurement tool to evaluate human cognitive status such as ability level and knowledge mastery. It has been applied to a wide range of fields including education, sport, psychological diagnosis, etc. By providing better awareness of cognitive status, it can serve as the basis for personalized services such as well-designed medical treatment, teaching strategy and vocational training. This paper aims to provide a survey of current models for cognitive diagnosis, with more attention on new developments using machine learning-based methods. By comparing the model structures, parameter estimation algorithms, model evaluation methods and applications, we provide a relatively comprehensive review of the recent trends in cognitive diagnosis models. Further, we discuss future directions that are worthy of exploration. In addition, we release two Python libraries: EduData for easy access to some relevant public datasets we have collected, and EduCDM that implements popular CDMs to facilitate both applications and research purposes.

==> TraditionalCD/main_backup_0606.tex <==
\section{Psychometrics-based Cognitive Diagnosis Models}  \label{sec:traditional_CD}
Traditional cognitive diagnosis models (CDMs) utilize statistical methods to model students' cognitive states. Along this line, traditional CDMs can be categorized into two paradigms, i.e., the \textit{ability level paradigm} and the \textit{cognition level paradigm}.

\begin{figure}[t]
    \centering
    % \includegraphics[width=1.0\textwidth]{TraditionalCD/traditional-cd.pdf}
    \begin{forest}
    for tree={
        scale=0.88,
        grow'=east,
        parent anchor=east,
        child anchor=west,
        anchor=west,   % left alignment for nodes
        edge path={  
            \noexpand\path [draw, \forestoption{edge}]  
            (!u.parent anchor) -- +(5pt,0) |- (.child anchor)\forestoption{edge label};  
        }, 
    }
    [Psychometrics-based\\ CDMs, draw, align=center  % , fill=yellow   keep align=center, or the line would not break
        [Ability level paradigm
            [IRT
                [Dichotomous IRT
                    [1PL/2PL/3PL-IRT]]
                [Polytomous IRT]
                [Other IRT models]
            ]
            [MIRT]
        ]
        [Cognition level paradigm
            [Rule Space Method]
            [{DINA, DINO, NIDA, NIDO, etc.}]
            [GDM]
            [Others
                [RUM]
                [LCDM]
                [MLTM-D]
                [...]
            ]
            
        ]
    ]
    \end{forest}
    \caption{A taxonomy of psychometrics-based cognitive diagnosis models}
    \label{fig:traditional-cd}
\end{figure}

\subsection{Ability Level Paradigm} \label{sec:ability_level}
\par In the ability level paradigm, researchers focus on the estimation of the \textit{overall ability} of students reflected on cognitive tests such as regular exams. Traditional CDMs following the ability level paradigm usually model students' overall abilities by low-dimensional parameters, which can be jointly estimated with low-dimensional item parameters such as discrimination and difficulty. Item Response Theory (IRT) \cite{Johns2006,Brzezinska2020} and Multidimensional Item Response Theory (MIRT) \cite{Reckase2009} are representative CDMs in this paradigm. 

\subsubsection{Item Response Theory} \label{sec:irt}
\par Item Response Theory (IRT) \cite{Johns2006,Brzezinska2020} models is a class of latent trait models for modeling students' cognitive states. The core assumption of IRT is that students' probabilities of correct response can be modeled by a continuous mathmatical function $f:\Theta\times\Psi\to[0,1]$, where $\Theta$ is the set of students' latent traits and $\Psi$ is the set of items' latent traits. The item response function $f$, also namely interaction function, essentially model the cognition process of students in answering an item.
In IRT, each student $i$'s latent trait is modeled by a scalar parameter $\theta_i$. Based on the modeling of item latent traits, IRT can be classified into one-parameter IRT (1PL-IRT), two-parameter IRT (2PL-IRT) and three-parameter IRT (3PL-IRT). In 1PL-IRT (also named as Rasch model \cite{ludlow1995rasch}), an item $j$ is modeled by its difficulty parameter $b_j$. Then the dichotomous response score $r_{ij}\in\{0,1\}$ is predicted by:
\begin{equation}
    Pr(r_{ij}=1 | \theta_i, b_j) = \frac{1}{1+e^{-(\theta_i-b_j)}},
\end{equation}
where $Pr(\cdot|\cdot)$ denotes conditional probability. 1PL-IRT is the simplest form of IRT and easy to deploy. However, 1PL-IRT fails to model more fine-grained attributes of items, which may highly affect students' performance in cognitive tests. To this end, researchers extend it to the 2PL-IRT model, which considers the significant \textit{discrimination} of different items. Specifically, let $a_j > 0$ denotes the discrimination parameter of item $j$, then the response score $r_{ij}$ is predicted by:

\begin{equation}
    Pr(r_{ij}=1 | \theta_i, a_j, b_j) = \frac{1}{1+e^{-a_j(\theta_i-b_j)}}.
\end{equation}

\par Moreover, based on 2PL-IRT, researchers proposed the 3PL-IRT, which introduces the \textit{guess} parameter of items to model students' item answering process more accurately:

\begin{equation}
    Pr(r_{ij}=1 | \theta_i, a_j, b_j, c_j) = c_j + (1-c_j)\frac{1}{1+e^{-a_j(\theta_i-b_j)}}.
\end{equation}

\par Despite IRT models model student ability in the simplest scalar form, their excellent mathematical properties (e.g., the convex property of the interaction function) endows them to be applied to a variety of downstream tasks such as computerized adaptive testing. In recent years, researchers also attempts to extend the usage of traditional IRT models. For instance, researchers developed various polytomous IRT models to address this issue, such as Partial Credit Rasch Model (PCM) \cite{Masters1982pcm}, Rating Scale Model (RSM) \cite{Andersen1997ratingsm} and Graded Response Model  (GRM) \cite{Samejima1969grm}. With the help of polytomous IRT models, users can get more accurate estimation of students' cognitive states.
 
\subsubsection{Multidimensional Item Response Theory}
\par Multidimensional Item Response Theory (MIRT) \cite{Reckase2009} extends student ability modelled in IRT to multidimensional cases, which enables mining students' cognitive states from various aspects. Similar to exploratory factor analysis (EFA),  MIRT allows for the exploration of multidimensionality and complex relationships between observed variables and latent traits, particularly in the context of assessments or tests. The simplest form of MIRT is given as follows:
\begin{equation}
    Pr(r_{ij}=1|\theta_i, a_j, b_j) = \frac{1}{1+e^{-(a_j^\top\theta_i+b_j)}},
\end{equation}
where $a_j$ denotes item discrimination on different dimensions, and $b_j$ denotes item difficulty on different dimensions. In real-world scenarios, each \textit{dimension} of $\theta_i$ represents a specific ability required to successfully answer the item, such as the mastery of specific knowledge concepts in course learning. To ensure the identifiability of MIRT, item discrimination vector $a_j$ of different items are usually rotated to the same value to acquire identifiable estimation of student abilities \cite{Béguin2001mirtfit}.
\par Besides relating to EFA and extending the dimension of IRT, MIRT also connects the cognition level paradigm. In the cognition level paradigm, researchers focus more on fine-grained cognitive states of students, such as proficiency level on different knowledge concepts, which helps students build their cognitive process. For instance,  da Silva et al. \cite{silva2019qmatrixmirt} introduce the Q-matrix (item-skill mapping matrix) into the interaction function of MIRT to obtain knowledge concept-wise student latent traits. 

\subsection{Cognition Level Paradigm}  \label{sec:cognition_level}
\par In the cognitive level paradigm, researchers focus on the estimation of the fine-grained cognitive states of students, which helps them build their cognitive process. For instance, in K-12 course learning, test designers require diagnosing students' proficiency level on knowledge concepts (e.g., the concept \textit{linear function} in mathematics) from their test performances. Therefore, cognitive level paradigm-based CDMs are utilized to estimate student knowledge proficiencies in this scenario. Since such a diagnosis process can be viewed as classifying students to an ``ideal'' proficiency pattern that is most suitable for his/her test performance, traditional cognitive level paradigm-based CDMs are also named as \textbf{Diagnostic Classification Model} (DCM).

\subsubsection{Rule Space Method (RSM) And Its Variations}
\par The rule space method (RSM), proposed by Tatsuoka in the 1980s \cite{tatsuoka1983rule}, is a statistical modeling approach used in educational measurement and cognitive diagnosis. The method is primarily applied in the context of IRT for modeling the relationship between individuals' latent traits and their responses to test items. The RSM focuses on representing the cognitive processes that individuals use to respond to test items. In traditional IRT models, the emphasis is on estimating the overall ability of an individual, but the RSM takes a more fine-grained approach. It seeks to identify the specific cognitive rules or strategies that individuals employ when answering test items. Specifically, cognitive diagnosis using RSM consists of five steps:
\begin{enumerate}
    \item \textbf{Item Decomposition}: Test items are decomposed into a set of rules or cognitive processes that are believed to be involved in successfully solving the item.
    \item \textbf{Rule Specification}: Each rule is defined explicitly in terms of binary knowledge proficiencies, which can be one-to-one mapped into an ideal response pattern. These rules represent the ways in which individuals can approach and solve the item.
    \item \textbf{Rule Space Construction}: The rule space is a multidimensional space where each dimension corresponds to a specific rule. Each point in this space represents a unique combination of rules that can be used to answer an item.
    \item \textbf{Rule Space Matching}: Individuals' response scores (response patterns) are utilized to calculate their similarity to ideal response patterns defined in rules. Then each individual is classified into the most similar rule, which reflect his/her cognitive states in the test.
\end{enumerate}

\par The RSM is a fundamental yet significant method in traditional CD, and is the basis of many DCMs \cite{leighton2004attribute,leighton2007cognitive}. One shortcoming of the traditional RSM is that it view knowledge concepts as independent entities and ignores their hierarchical relationship in students' cognitive process (e.g., knowledge dependency). Therefore, Leighton et al. \cite{leighton2004attribute} proposed the Attribute Hierarchy Method (AHM) to address this issue. Compared to the original RSM, the AHM assumes that attributes (i.e., knowledge concepts or skills that are required for students to solve a test item) are organized in a hierarchical structure, which can be represented by an adjacent matrix of attributes. Then the AHM limits the rule space defined in the RSM, such that the mastery of any child attribute should be no less than the mastery of its parent attribute. Then the AHM match each student into the most similar ideal response patterns, with the corresponding rule as the diagnostic result of the student.

\subsubsection{DINA And Relevant DCMs}
\par Deterministic Input, Noisy ``And'' Gate (DINA) model \cite{de2009dina} and relevant DCMs focus on diagnosing students' knowledge concept-wise abilities from binary response data and expert-labeled question-knowledge relationship. Each of them utilizes a continuous mathematical function to model the relationship between probabilities of students' correct response and their latent knowledge proficiency.  The core assumption of DINA is that the proficiency of different knowledge concepts is \textbf{non-compensatory}. That is, the model assumes that mastery of all required attributes is necessary for a correct response, but also allow for the possibility of guessing. In DINA, each student $i$'s cognitive state is modelled as his/her binary knowledge proficiency levels on each knowledge concepts, which can be represented by a $K$-dimensional binary 0-1 vector $\theta_i = (\theta_{i1},\ldots,\theta_{iK})$. Here $K$ denotes the number of knowledge concepts, and the binary value $\theta_{ik}$ denotes student $i$'s proficiency level of concept $k$. Item are modelled by ``slip'' and ``guess'' parameters and a pre-given binary \textbf{Q-matrix} $Q = (q_1, \ldots, q_J)^\top = (q_{jk})_{J\times K}$, where the binary value $q_{jk}$ denotes whether item $j$ requires knowledge concept $k$. Next, the interaction function of DINA is defined as follows:

\begin{equation}
    Pr(r_{ij}=1|\theta_i,q_j, s_j, g_j) = (1-s_j)^{\eta_{ij}}g_j^{1-\eta_{ij}},
\end{equation}
where $\eta_{ij} = \prod_{k=1}^{K}\theta_{ik}^{q_{jk}}$ is the indicator of whether the student has mastered \textit{all} required knowledge concepts of the item. The $s_j$ and $g_j$ denote respectively the ``slip'' and ``guess'' parameters of item $j$. Then the goal of the DINA model is to estimate student cognitive state $\theta_i$ and item parameters $s_j$ and $g_j$ given observed binary response scores.
\par On the other hand, the Deterministic Input, Noisy ``Or'' Gate (DINO) model \cite{templin2006dino} is a representative \textbf{compensatory} model. That is to say, the proficiency of different knowledge concepts is \textbf{compensatory} in DINO. Specifically, DINO assume that each item requires a certain level of proficiency on each attribute, and performance on each attribute contributes additively to the probability of a correct response. Compare to DINA, DINO has a more flexible and relaxed requirement for students' knowledge proficiency to correct answer a question. The compensatory assumption is more consistent with students' cognitive process in real-world scenarios. However, DINO suffers from the risk of over-estimation of students' ability due to the compensatory assumption, and the parameter estimation of DINA is more complex.
\par Noisy Inputs, Deterministic "And" Gate (NIDA) model \cite{maris1999nida} and Noisy Inputs, Deterministic "Or" Gate (NIDO) model are also DCMs relevant to DINA and DINO. Different from DINA and DINO, NIDA and NIDO models assume that there might exit noise in students' knowledge proficiencies. Based on this assumption, NIDA is a non-compensatory DCM like DINA, while NIDO is a compensatory DCM like DINO. In a word, DINA and its relevant DCMs can be categorized as shown in Table \ref{tab:category-dina}.

\begin{table}[htp]
\caption{A categorization of DINA and its relevant DCMs.}
\label{tab:category-dina}
\begin{tabular}{l|l|l}
\hline
\textbf{DCM} & \textbf{Non-compensatory} & \textbf{Compensatory} \\ \hline
\textbf{Deterministic knowledge proficiency} & DINA \cite{de2009dina} & DINO \cite{templin2006dino} \\ \hline
\textbf{Noisy knowledge proficiency} & NIDA \cite{maris1999nida} & NIDO \cite{templin2006dino} \\ \hline
\end{tabular}
\end{table}

% \par The DINA model has many beneficial characteristics. First, DINA is a lightweight model because it only models each item by two parameters, and there does not exist any inner parameter in the interaction function, which is common in deep learning models. Second, DINA is a \textit{non-compensatory} DCM, because the definition of the ideal response $\eta_{ij}$ requires that students have to mastery \textit{all required knowledge concepts} to correctly respond to the item, and the mastery of a knowledge concept cannot compensate for the non-mastery of another. In addition, the term ``deterministic input'' in DINA means that the ideal response $\eta_{ij}$ is completely determined by student cognitive states $\theta_i$ and item Q vector $q_j$, while the ``noisy output'' in DINA means that the correct response probability is also affected by noisy factors, i.e., the slip and guess behaviors of students. Due to its advantages in modelling student cognitive states and simulating student response patterns, DINA has gain more and more attention by researchers in the area of cognitive diagnosis and educational measurement. 

\subsubsection{General Diagnostic Model (GDM)}
\par As reflected on its name, the General Diagnostic Model (GDM) \cite{vondavier2005gdm} is a general framework that subsumes many classical and well-known CDMs like DINA, IRT and MIRT \cite{vondavier2014gdm, bradshaw2014gdm}. As a general framework, GDM is suitable for various real-world scenarios, including but not limited to dichotomous / polytomous response scores, binary / continuous / polytomous ordinal knowledge mastery levels, etc. For simplicity, we introduce GDM for binary and ordinal skill profiles in this section.
\par Formally, let $\theta = (\theta_1, \ldots, \theta_D)$ be a D-dimensional skill profile consisting of polytomous or dichotomous skill attributes $\theta_d, d = 1,\ldots, D$. Then the probability of a polytomous response score $x\in\{0,\ldots,m_i\}$ to item $j$ under the GDM with an individual with skill profiles $\theta$ is defined as

\begin{equation}
    P(X_j = x|\theta = (\theta_1,\ldots,\theta_D)) = \frac{\exp\left[\beta_{jx} + \sum_{d=1}^{D}\gamma_{jxd}h_j(q_{jd},\theta_d)\right]}{1+\sum_{y=1}^{m_j}\exp\left[\beta_{jy} + \sum_{d=1}^{D}\gamma_{jyd}h_j(q_{jd},\theta_d)\right]},
\end{equation}
where $\beta_{jx},\gamma_{jxd}, j = 1,2,\ldots,J, x = 1,2,\ldots,m_j, d = 1,2,\ldots D$ are estimable item parameters. Each element $q_{jd}, j = 1,2,\ldots J, d = 1,2,\ldots, D$ of the Q-matrix is a constant, as in other DCMs like DINA. The helper function $h(\cdot,\cdot)$ map $q_{jd}$ and $\theta_d$ to a real number, which considers the fact that the knowledge profile $\theta$ might be polytomous.
\par The implementation of GDM is divided into two classes: GDM for polytomous data and GDM for binary data. For polytomous data, the term $\gamma_{jxd}$ is implemented as $\gamma_{jxd} = x\gamma_{jd}$, where $x$ denotes the polytomous score. The helper function is implemented as $h_j(q_{jd},\theta_d) = q_{jd}\theta_d$. Then the interaction function is implemented as follows:
\begin{equation}
    P(X_j = x|\theta = (\theta_1,\ldots,\theta_D)) = \frac{\exp\left[\beta_{jx} + \sum_{d=1}^{D}x\gamma_{jd}q_{jd}\theta_d\right]}{1+\sum_{y=1}^{m_j}\exp\left[\beta_{jy} + \sum_{d=1}^{D}y\gamma_{jd}q_{jd}\theta_d\right]}.
\end{equation}
\par Similarly for binary response data, the interaction function reduces to
\begin{equation}
    P(X_j = x|\theta = (\theta_1,\ldots,\theta_D)) = \frac{\exp\left[\beta_{jx} + \sum_{d=1}^{D}\gamma_{jd}q_{jd}\theta_d\right]}{1+\sum_{y=1}^{m_j}\exp\left[\beta_{jy} + \sum_{d=1}^{D}\gamma_{jd}q_{jd}\theta_d\right]}.
\end{equation}
\par In terms of parameter estimation, as a constraint latent class model, the parameter estimation of GDM is usually done with expectation-maximization (EM) algorithm \cite{dempster1977em,huo2014em}. Compare to other estimation algorithms, the EM algorithm for GDM is more suitable for large-scale data and data with missing values, which makes it flexible to complex real-world scenarios.
\par Due to its generality and flexibility, there are also many other versions for GDM to adjust some special scenarios, like mixture distribution extensions of GDM which considers the ability prior of student groups, and  hierarchical extensions of GDM which consider the multilevel distribution of student abilities. Indeed, many traditional CDMs, including CDMs in the ability level paradigm like IRT and MIRT \cite{bradshaw2014gdm}, and CDMs in the cognitive level paradigm like LCDM and DINA \cite{vondavier2014gdm}, have been proved to be special cases of GDM. 

\subsubsection{Other Traditional CDMs}
\par Besides representative CDMs introduced above, there are also some other traditional CDMs that focus on different research challenges in the context of educational measurement. For instance, the Reparameterized Unified Model (RUM) \cite{hartz2002rum}, as a refinement of DINA, aims to construct a cognitive diagnosis assessment system that includes DCM models, estimation procedure, classification algorithm and model-and-data checking function. De La Torre \cite{de2011generalized} proposed the G-DINA, as a general cognitive diagnosis framework similar to GDM, which subsumes many existing CDMs like DINA. Henson et al. \cite{henson2009lcdm} proposed the Log-Linear Cognitive Diagnosis Model (LCDM), which is a flexble and general cognitive diagnosis model that can be directly tied to general log-linear model for the use of a multiple-way ANOVA and does not require user-specified relationship between attributes and the probability of a correct response. LCDM is also a special case of GDM which focus more on the interaction between students and items \cite{vondavier2014lcdm}. Embretson and Yang \cite{embretson2013mltmd} proposed the Multicomponent Latent Trait Model for Diagnosis (MLTM-D), which aims to diagnose hierarchically-structured skills or knowledge concepts. In a word, traditional CDMs are usually based on statistical models, and can be applied to a variety of real-world cognitive diagnosis scenarios. However, these models are hard to handle large-scale response data, where the time complexity of the parameter estimation algorithm is the main bottleneck. 
